Grid-Forming Control Methods for Weakly Connected Offshore WPPs

Grid-forming control (GFC) has seen numerous technological advances in their control types, applications, and the multitude of services they provide. Some examples of the services they provide include black start, inertial frequency response, and islanded operation capabilities with the possibility of re-synchronization without the need of additional support from other devices such as storage. State of the art literature proposes a variety of GFCs which can provide single or multiple of these services. However, study of these different GFCs for weakly-connected offshore wind power plants (WPPs) based on time-domain simulation and focusing on the large signal disturbance is not well covered. This paper reviews some of the most researched grid-forming control methods applicable to offshore WPPs and provides a comparative investigation and discussion of their stability properties and applicability, especially when connected to a weak-grid. The paper also provides a discussion on the prerequisites and challenges surrounding the comparative study of different GFCs.

==> bibliography.tex <==
@article{GBGFSpecs,
  title={GC0137: Minimum Specification Required for Provision of GB Grid Forming (GBGF) Capability (formerly Virtual Synchronous Machine/VSM Capability)},
  author={Workgroup Consultation GC0137},
  year={2021},
  publisher={NationalGridESO}
}

@article{DGC325,
  title={Classification: Offentlig/Public Technical regulation 3.2.5 for wind power plants above 11 kW},
  author={Energinet},
  year={2016},
  publisher={Energinet}
}

@techreport{lin2020research,
  title={Research roadmap on grid-forming inverters},
  author={Lin, Yashen and Eto, Joseph H and Johnson, Brian B and Flicker, Jack D and Lasseter, Robert H and Villegas Pico, Hugo N and Seo, Gab-Su and Pierre, Brian J and Ellis, Abraham},
  year={2020},
  institution={National Renewable Energy Lab.(NREL), Golden, CO (United States)}
}

@article{cunha2021generalized,
  title={Generalized Formulation of Steady-State Equivalent Circuit Models of Grid-Forming Inverters},
  author={Cunha, Vinicius C and Kim, Taehyung and Barry, Nicholas and Siratarnsophon, Piyapath and Santoso, Surya and Freitas, Walmir and Ramasubramanian, Deepak and Dugan, Roger C},
  journal={IEEE Open Access Journal of Power and Energy},
  volume={8},
  pages={352--364},
  year={2021},
  publisher={IEEE}
}

@article{sinha2015uncovering,
  title={Uncovering droop control laws embedded within the nonlinear dynamics of van der pol oscillators},
  author={Sinha, Mohit and D{\"o}rfler, Florian and Johnson, Brian B and Dhople, Sairaj V},
  journal={IEEE Transactions on Control of Network Systems},
  volume={4},
  number={2},
  pages={347--358},
  year={2015},
  publisher={IEEE}
}

@INPROCEEDINGS{8722028,
  author={Seo, Gab-Su and Colombino, Marcello and Subotic, Irina and Johnson, Brian and Groß, Dominic and Dörfler, Florian},
  booktitle={2019 IEEE Applied Power Electronics Conference and Exposition (APEC)}, 
  title={Dispatchable Virtual Oscillator Control for Decentralized Inverter-dominated Power Systems: Analysis and Experiments}, 
  year={2019},
  volume={},
  number={},
  pages={561-566},
  doi={10.1109/APEC.2019.8722028}}

@article{chen2020modelling,
  title={Modelling, implementation, and assessment of virtual synchronous generator in power systems},
  author={Chen, Meng and Zhou, Dao and Blaabjerg, Frede},
  journal={Journal of Modern Power Systems and Clean Energy},
  volume={8},
  number={3},
  pages={399--411},
  year={2020},
  publisher={SGEPRI}
}

@article{park1929two,
  title={Two-reaction theory of synchronous machines generalized method of analysis-part I},
  author={Park, Robert H},
  journal={Transactions of the American Institute of Electrical Engineers},
  volume={48},
  number={3},
  pages={716--727},
  year={1929},
  publisher={IEEE}
}

@article{pogaku2007modeling,
  title={Modeling, analysis and testing of autonomous operation of an inverter-based microgrid},
  author={Pogaku, Nagaraju and Prodanovic, Milan and Green, Timothy C},
  journal={IEEE Transactions on power electronics},
  volume={22},
  number={2},
  pages={613--625},
  year={2007},
  publisher={IEEE}
}

@article{tayyebi2019interactions,
  title={Interactions of grid-forming power converters and synchronous machines},
  author={Tayyebi, Ali and Gro{\ss}, Dominic and Anta, Adolfo and Kupzog, Friederich and D{\"o}rfler, Florian},
  journal={arXiv preprint arXiv:1902.10750},
  year={2019}
}

@ARTICLE{8242351,  author={Adib, Aswad and Mirafzal, Behrooz and Wang, Xiongfei and Blaabjerg, Frede},  journal={IEEE Access},   title={On Stability of Voltage Source Inverters in Weak Grids},   year={2018},  volume={6},  number={},  pages={4427-4439},  doi={10.1109/ACCESS.2017.2788818}}

@ARTICLE{7776920,  author={Li, Zhongwen and Zang, Chuanzhi and Zeng, Peng and Yu, Haibin and Li, Shuhui and Bian, Jing},  journal={IEEE Transactions on Industrial Electronics},   title={Control of a Grid-Forming Inverter Based on Sliding-Mode and Mixed ${H_2}/{H_\infty }$ Control},   year={2017},  volume={64},  number={5},  pages={3862-3872},  doi={10.1109/TIE.2016.2636798}}

@ARTICLE{993176,  author={Coelho, E.A.A. and Cortizo, P.C. and Garcia, P.F.D.},  journal={IEEE Transactions on Industry Applications},   title={Small-signal stability for parallel-connected inverters in stand-alone AC supply systems},   year={2002},  volume={38},  number={2},  pages={533-542},  doi={10.1109/28.993176}}

@ARTICLE{6891273,  author={D'Arco, Salvatore and Suul, Jon Are and Fosso, Olav Bjarte},  journal={IEEE Transactions on Industry Applications},   title={Automatic Tuning of Cascaded Controllers for Power Converters Using Eigenvalue Parametric Sensitivities},   year={2015},  volume={51},  number={2},  pages={1743-1753},  doi={10.1109/TIA.2014.2354732}}

@book{utkin2017sliding,
  title={Sliding mode control in electro-mechanical systems},
  author={Utkin, Vadim and Guldner, J{\"u}rgen and Shi, Jingxin},
  year={2017},
  publisher={CRC press}
}

@ARTICLE{9513281,  author={Rathnayake, Dayan B. and Akrami, Milad and Phurailatpam, Chitaranjan and Me, Si Phu and Hadavi, Sajjad and Jayasinghe, Gamini and Zabihi, Sasan and Bahrani, Behrooz},  journal={IEEE Access},   title={Grid Forming Inverter Modeling, Control, and Applications},   year={2021},  volume={9},  number={},  pages={114781-114807},  doi={10.1109/ACCESS.2021.3104617}}

@INPROCEEDINGS{8450880,  author={Milano, Federico and Dörfler, Florian and Hug, Gabriela and Hill, David J. and Verbič, Gregor},  booktitle={2018 Power Systems Computation Conference (PSCC)},   title={Foundations and Challenges of Low-Inertia Systems (Invited Paper)},   year={2018},  volume={},  number={},  pages={1-25},  doi={10.23919/PSCC.2018.8450880}}

@article{kundur2004definition,
  title={Definition and classification of power system stability IEEE/CIGRE joint task force on stability terms and definitions},
  author={Kundur, Prabha and Paserba, John and Ajjarapu, Venkat and Andersson, G{\"o}ran and Bose, Anjan and Canizares, Claudio and Hatziargyriou, Nikos and Hill, David and Stankovic, Alex and Taylor, Carson and others},
  journal={IEEE transactions on Power Systems},
  volume={19},
  number={3},
  pages={1387--1401},
  year={2004},
  publisher={IEEE}
}

@article{kkuni2021effects,
  title={Effects of current limit for grid forming converters on transient stability: analysis and solution},
  author={Kkuni, Kanakesh Vatta and Yang, Guangya},
  journal={arXiv preprint arXiv:2106.13555},
  year={2021}
}

@article{ratnam2020future,
  title={Future low-inertia power systems: Requirements, issues, and solutions-A review},
  author={Ratnam, Kamala Sarojini and Palanisamy, K and Yang, Guangya},
  journal={Renewable and Sustainable Energy Reviews},
  volume={124},
  pages={109773},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{van2010virtual,
  title={Virtual synchronous generator: An element of future grids},
  author={Van, T Vu and Visscher, Klaas and Diaz, Javier and Karapanos, Vasileios and Woyte, Achim and Albu, M and Bozelie, Jan and Loix, Tom and Federenciuc, Dumitru},
  booktitle={2010 IEEE PES Innovative Smart Grid Technologies Conference Europe (ISGT Europe)},
  pages={1--7},
  year={2010},
  organization={IEEE}
}

@inproceedings{visscher2008virtual,
  title={Virtual synchronous machines (VSG’s) for frequency stabilisation in future grids with a significant share of decentralized generation},
  author={Visscher, Klaas and De Haan, Sjoerd Walter Hero},
  booktitle={CIRED Seminar 2008: SmartGrids for Distribution},
  pages={1--4},
  year={2008},
  organization={IET}
}

@inproceedings{wang2015synchronous,
  title={Synchronous frequency resonance of virtual synchronous generators and damping control},
  author={Wang, Jinhua and Wang, Yuxiang and Gu, Yunjie and Li, Wuhua and He, Xiangning},
  booktitle={2015 9th International Conference on Power Electronics and ECCE Asia (ICPE-ECCE Asia)},
  pages={1011--1016},
  year={2015},
  organization={IEEE}
}

@inproceedings{ierna2016effects,
  title={Effects of VSM Convertor Control on Penetration Limits of Non-Synchronous Generation in the GB Power System},
  author={Ierna, Richard and Roscoe, Andrew and Yu, Meng and Urdal, Helge and Dy{\'s}ko, Andrzej and et al.},
  booktitle={15th Wind Integration Workshop},
  year={2016},
  address={Vienna}
}

@ARTICLE{7781612,
  author={Mo, Olve and D'Arco, Salvatore and Suul, Jon Are},
  journal={IEEE Transactions on Industrial Electronics}, 
  title={Evaluation of Virtual Synchronous Machines With Dynamic or Quasi-Stationary Machine Models}, 
  year={2017},
  volume={64},
  number={7},
  pages={5952-5962},
  doi={10.1109/TIE.2016.2638810}}

@INPROCEEDINGS{9092640,
  author={Liao, Yicheng and Wang, Xiongfei and Liu, Fangcheng and Xin, Kai and Liu, Yunfeng},
  booktitle={2019 4th IEEE Workshop on the Electronic Grid (eGRID)}, 
  title={Sub-Synchronous Control Interaction in Grid-Forming VSCs with Droop Control}, 
  year={2019},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/eGRID48402.2019.9092640}}

@inproceedings{roscoe2016vsm,
  author = {Roscoe, A. J. and Yu, M. and Ierna, R. and Zhu, J. and Dysko, A. and Urdal, H. and et al.},
  title = {A VSM (Virtual Synchronous Machine) Convertor Control Model Suitable for RMS Studies for Resolving System Operator/Owner Challenges},
  booktitle = {15th Wind Integration Workshop},
  year = {2016}
}


@INPROCEEDINGS{9281712,
  author={Pattabiraman, Dinesh and Lasseter, Robert H. and Jahns, Thomas M.},
  booktitle={2020 IEEE Power & Energy Society General Meeting (PESGM)}, 
  title={Transient Stability Modeling of Droop-Controlled Grid-Forming Inverters with Fault Current Limiting}, 
  year={2020},
  volume={},
  number={},
  pages={1-5},
  doi={10.1109/PESGM41954.2020.9281712}}

@inproceedings{van2009grid,
  title={Grid tied converter with virtual kinetic storage},
  author={Van Wesenbeeck, MPN and De Haan, SWH and Varela, Pablo and Visscher, Klaas},
  booktitle={2009 IEEE Bucharest PowerTech},
  pages={1--7},
  year={2009},
  organization={IEEE}
}

@article{musca2022grid,
  title={Grid-forming converters. A critical review of pilot projects and demonstrators},
  author={Musca, Rossano and Vasile, Antony and Zizzo, Gaetano},
  journal={Renewable and Sustainable Energy Reviews},
  volume={165},
  pages={112551},
  year={2022},
  publisher={Elsevier}
}

@article{tielens2016relevance,
  title={The relevance of inertia in power systems},
  author={Tielens, Pieter and Van Hertem, Dirk},
  journal={Renewable and Sustainable Energy Reviews},
  volume={55},
  pages={999--1009},
  year={2016},
  publisher={Elsevier}
}

@article{heylen2021challenges,
  title={Challenges and opportunities of inertia estimation and forecasting in low-inertia power systems},
  author={Heylen, Evelyn and Teng, Fei and Strbac, Goran},
  journal={Renewable and Sustainable Energy Reviews},
  volume={147},
  pages={111176},
  year={2021},
  publisher={Elsevier}
}

@article{roscoe2020response,
  title={Response of a grid forming wind farm to system events, and the impact of external and internal damping},
  author={Roscoe, Andrew and Knueppel, Thyge and Da Silva, Ricardo and Brogan, Paul and Gutierrez, Isaac and Elliott, Douglas and Perez Campion, Juan-Carlos},
  journal={IET Renewable Power Generation},
  volume={14},
  number={19},
  pages={3908--3917},
  year={2020},
  publisher={Wiley Online Library}
}

@article{wang2017stability,
  title={Stability analysis and controller synthesis for single-loop voltage-controlled VSIs},
  author={Wang, Xiongfei and Loh, Poh Chiang and Blaabjerg, Frede},
  journal={IEEE Transactions on Power Electronics},
  volume={32},
  number={9},
  pages={7394--7404},
  year={2017},
  publisher={IEEE}
}

@article{geng2017parameters,
  title={Parameters design and optimization for LC-type off-grid inverters with inductor-current feedback active damping},
  author={Geng, Yiwen and Yun, Yang and Chen, Ruicheng and Wang, Kai and Bai, Haofeng and Wu, Xiaojie},
  journal={IEEE Transactions on Power Electronics},
  volume={33},
  number={1},
  pages={703--715},
  year={2017},
  publisher={IEEE}
}

@article{liao2020passivity,
  title={Passivity-based analysis and design of linear voltage controllers for voltage-source converters},
  author={Liao, Yicheng and Wang, Xiongfei and Blaabjerg, Frede},
  journal={IEEE Open Journal of the Industrial Electronics Society},
  volume={1},
  pages={114--126},
  year={2020},
  publisher={IEEE Press}
}

@article{zhang2009power,
  title={Power-synchronization control of grid-connected voltage-source converters},
  author={Zhang, Lidong and Harnefors, Lennart and Nee, Hans-Peter},
  journal={IEEE Transactions on Power systems},
  volume={25},
  number={2},
  pages={809--820},
  year={2009},
  publisher={IEEE}
}

@article{harnefors2015passivity,
  title={Passivity-based stability assessment of grid-connected VSCs—An overview},
  author={Harnefors, Lennart and Wang, Xiongfei and Yepes, Alejandro G and Blaabjerg, Frede},
  journal={IEEE Journal of emerging and selected topics in Power Electronics},
  volume={4},
  number={1},
  pages={116--125},
  year={2015},
  publisher={IEEE}
}

@ARTICLE{9751441,
  author={Song, Guanhong and Cao, Bo and Chang, Liuchen},
  journal={Chinese Journal of Electrical Engineering}, 
  title={Review of Grid-forming Inverters in Support of Power System Operation}, 
  year={2022},
  volume={8},
  number={1},
  pages={1-15},
  doi={10.23919/CJEE.2022.000001}}

@INPROCEEDINGS{9759663,
  author={Zhang, Guangdou and Li, Jian and Xing, Yankai and Bamisile, Olusola and Huang, Qi},
  booktitle={2022 4th Asia Energy and Electrical Engineering Symposium (AEEES)}, 
  title={Grid-Forming Converter in High Penetration of Converter-Interfaced Generation Large-Scale Power System: A Review of Synchronization Stability}, 
  year={2022},
  volume={},
  number={},
  pages={967-973},
  doi={10.1109/AEEES54426.2022.9759663}}

@ARTICLE{9408354,
  author={Rosso, Roberto and Wang, Xiongfei and Liserre, Marco and Lu, Xiaonan and Engelken, Soenke},
  journal={IEEE Open Journal of Industry Applications}, 
  title={Grid-Forming Converters: Control Approaches, Grid-Synchronization, and Future Trends—A Review}, 
  year={2021},
  volume={2},
  number={},
  pages={93-109},
  doi={10.1109/OJIA.2021.3074028}}

@ARTICLE{9627884,
  author={Zhang, Haobo and Xiang, Wang and Lin, Weixing and Wen, Jinyu},
  journal={Journal of Modern Power Systems and Clean Energy}, 
  title={Grid Forming Converters in Renewable Energy Sources Dominated Power Grid: Control Strategy, Stability, Application, and Challenges}, 
  year={2021},
  volume={9},
  number={6},
  pages={1239-1256},
  doi={10.35833/MPCE.2021.000257}}

@ARTICLE{6200347,
  author={Rocabert, Joan and Luna, Alvaro and Blaabjerg, Frede and Rodríguez, Pedro},
  journal={IEEE Transactions on Power Electronics}, 
  title={Control of Power Converters in AC Microgrids}, 
  year={2012},
  volume={27},
  number={11},
  pages={4734-4749},
  doi={10.1109/TPEL.2012.2199334}}

@INPROCEEDINGS{9236314,
  author={Rosso, Roberto and Engelken, Soenke and Liserre, Marco},
  booktitle={2020 IEEE Energy Conversion Congress and Exposition (ECCE)}, 
  title={Current Limitation Strategy For Grid-Forming Converters Under Symmetrical And Asymmetrical Grid Faults}, 
  year={2020},
  volume={},
  number={},
  pages={3746-3753},
  doi={10.1109/ECCE44975.2020.9236314}}

@ARTICLE{8495031,
  author={Wu, Heng and Wang, Xiongfei},
  journal={IEEE Transactions on Industrial Electronics}, 
  title={Design-Oriented Transient Stability Analysis of Grid-Connected Converters With Power Synchronization Control}, 
  year={2019},
  volume={66},
  number={8},
  pages={6473-6482},
  doi={10.1109/TIE.2018.2875669}}

@article{matevosyan2019grid,
  title={Grid-forming inverters: Are they the key for high renewable penetration?},
  author={Matevosyan, Julia and Badrzadeh, Babak and Prevost, Thibault and Quitmann, Eckard and Ramasubramanian, Deepak and Urdal, Helge and Achilles, Sebastian and MacDowell, Jason and Huang, Shun Hsien and Vital, Vijay and others},
  journal={IEEE Power and Energy magazine},
  volume={17},
  number={6},
  pages={89--98},
  year={2019},
  publisher={IEEE}
}

@inproceedings{ndreko2018grid,
  title={Grid forming control for stable power systems with up to 100\% inverter based generation: a paradigm scenario using the IEEE 118-bus system},
  author={Ndreko, Mario and R{\"u}berg, Sven and Winter, Wilhelm},
  booktitle={Proceedings of the 17th International Wind Integration Workshop, Stockholm, Sweden},
  pages={16--18},
  year={2018}
}

@article{marinakis2021grid,
  title={Grid forming control for power systems with up to 100\% inverter based generation},
  author={Marinakis, Panagiotis and Schofield, Nigel},
  year={2021},
  publisher={IET}
}

@article{pawar2021grid,
  title={Grid-forming control for solar PV systems with power reserves},
  author={Pawar, Bandopant and Batzelis, Efstratios I and Chakrabarti, Saikat and Pal, Bikash C},
  journal={IEEE Transactions on Sustainable Energy},
  volume={12},
  number={4},
  pages={1947--1959},
  year={2021},
  publisher={IEEE}
}

@article{singh2015grid,
  title={Grid forming Battery Energy Storage System (BESS) for a highly unbalanced hybrid mini-grid},
  author={Singh, Maninder and Lopes, Luiz AC and Ninad, Nayeem A},
  journal={Electric Power Systems Research},
  volume={127},
  pages={126--133},
  year={2015},
  publisher={Elsevier}
}

@article{jain2020grid,
  title={Grid-forming control strategies for black start by offshore wind power plants},
  author={Jain, Anubhav and Sakamuri, Jayachandra N and Cutululis, Nicolaos A},
  journal={Wind Energy Science},
  volume={5},
  number={4},
  pages={1297--1313},
  year={2020},
  publisher={Copernicus GmbH}
}

@misc{IEA2022,
  author = {{IEA}},
  title = {Wind Electricity},
  year = {2022},
  howpublished = {{IEA}},
  note = {License: CC BY 4.0},
  url = {https://www.iea.org/reports/wind-electricity}
}

@article{dong2018small,
  title={Small signal stability analysis of multi-infeed power electronic systems based on grid strength assessment},
  author={Dong, Wei and Xin, Huanhai and Wu, Di and Huang, Linbin},
  journal={IEEE transactions on Power Systems},
  volume={34},
  number={2},
  pages={1393--1403},
  year={2018},
  publisher={IEEE}
}

@INPROCEEDINGS{6634621,
  author={Rodriguez, Pedro and Candela, Ignacio and Citro, Costantino and Rocabert, Joan and Luna, Alvaro},
  booktitle={2013 15th European Conference on Power Electronics and Applications (EPE)}, 
  title={Control of grid-connected power converters based on a virtual admittance control loop}, 
  year={2013},
  volume={},
  number={},
  pages={1-10},
  doi={10.1109/EPE.2013.6634621}}

@ARTICLE{1490703,
  author={Guerrero, J.M. and Luis Garcia de Vicuna and Matas, J. and Castilla, M. and Miret, J.},
  journal={IEEE Transactions on Industrial Electronics}, 
  title={Output impedance design of parallel-connected UPS inverters with wireless load-sharing control}, 
  year={2005},
  volume={52},
  number={4},
  pages={1126-1135},
  doi={10.1109/TIE.2005.851634}}

@INPROCEEDINGS{10131594,
  author={Zhao, Liang and Wang, Xiongfei and Gong, Hong and Jin, Zheming},
  booktitle={2023 IEEE Applied Power Electronics Conference and Exposition (APEC)}, 
  title={Stability Impact of Hybrid Synchronization Strategy on Virtual-Admittance-Based Grid-Forming Inverters}, 
  year={2023},
  volume={},
  number={},
  pages={2735-2740},
  doi={10.1109/APEC43580.2023.10131594}}

@ARTICLE{7052341,
  author={Kuperman, Alon},
  journal={IEEE Transactions on Power Electronics}, 
  title={Proportional-Resonant Current Controllers Design Based on Desired Transient Performance}, 
  year={2015},
  volume={30},
  number={10},
  pages={5341-5345},
  doi={10.1109/TPEL.2015.2408053}}

@ARTICLE{7446308,
  author={de Bosio, Federico and de Souza Ribeiro, Luiz Antonio and Freijedo, Francisco D. and Pastorelli, Michele and Guerrero, Josep M.},
  journal={IEEE Transactions on Industrial Electronics}, 
  title={Effect of State Feedback Coupling and System Delays on the Transient Performance of Stand-Alone VSI With LC Output Filter}, 
  year={2016},
  volume={63},
  number={8},
  pages={4909-4918},
  doi={10.1109/TIE.2016.2549990}}

@ARTICLE{9194347,
  author={Quan, Xiangjun},
  journal={IEEE Transactions on Industrial Electronics}, 
  title={Improved Dynamic Response Design for Proportional Resonant Control Applied to Three-Phase Grid-Forming Inverter}, 
  year={2021},
  volume={68},
  number={10},
  pages={9919-9930},
  doi={10.1109/TIE.2020.3021654}}

@INPROCEEDINGS{6736685,
  author={Dhople, Sairaj V. and Johnson, Brian B. and Hamadeh, Abdullah O.},
  booktitle={2013 51st Annual Allerton Conference on Communication, Control, and Computing (Allerton)}, 
  title={Virtual Oscillator Control for voltage source inverters}, 
  year={2013},
  volume={},
  number={},
  pages={1359-1363},
  doi={10.1109/Allerton.2013.6736685}}

@ARTICLE{8638531,
  author={Colombino, Marcello and Groß, Dominic and Brouillon, Jean-Sébastien and Dörfler, Florian},
  journal={IEEE Transactions on Automatic Control}, 
  title={Global Phase and Magnitude Synchronization of Coupled Oscillators With Application to the Control of Grid-Forming Power Inverters}, 
  year={2019},
  volume={64},
  number={11},
  pages={4496-4511},
  doi={10.1109/TAC.2019.2898549}}

@ARTICLE{8732453,
  author={Groß, Dominic and Colombino, Marcello and Brouillon, Jean-Sébastien and Dörfler, Florian},
  journal={IEEE Transactions on Control of Network Systems}, 
  title={The Effect of Transmission-Line Dynamics on Grid-Forming Dispatchable Virtual Oscillator Control}, 
  year={2019},
  volume={6},
  number={3},
  pages={1148-1160},
  doi={10.1109/TCNS.2019.2921347}}


@article{PLLInstAmir,
title = {PLL Instability of Wind Turbines during Severe Faults},
keywords = {Adaptive-PLL, Estimated impedance value, Grid following wind turbines, Loss of synchronisation, PLL instability, Severe faults},
author = {Amir Arasteh and Cutululis, {Nicolaos A.}},
year = {2022},
language = {English},
volume = {10},
pages = {4495--4505},
journal = {IEEE Access},
issn = {2169-3536},
publisher = {Institute of Electrical and Electronics Engineers}
}

@mastersthesis{ghimire2021dynamics,
  title={Dynamics and Stability of Inverter Dominated Low Inertia Power Grids},
  author={Ghimire, Sulav},
  year={2021},
  school={Skolkovo Institute of Science and Technology, Moscow, Russian Federation}
}

@INPROCEEDINGS{7897172,
  author={Masaud, Tarek Medalel and Mistry, Ronak Deepak},
  booktitle={2016 IEEE Conference on Technologies for Sustainability (SusTech)}, 
  title={Fault current contribution of Renewable Distributed Generation: An overview and key issues}, 
  year={2016},
  volume={},
  number={},
  pages={229-234},
  doi={10.1109/SusTech.2016.7897172}}

